"I Never Said That": A dataset, taxonomy and baselines on response clarity classification

Equivocation and ambiguity in public speech are well-studied discourse phenomena, especially in political science and analysis of political interviews. Inspired by the well-grounded theory on equivocation, we aim to resolve the closely related problem of response clarity in questions extracted from political interviews, leveraging the capabilities of Large Language Models (LLMs) and human expertise. To this end, we introduce a novel taxonomy that frames the task of detecting and classifying response clarity and a corresponding clarity classification dataset which consists of question-answer (QA) pairs drawn from political interviews and annotated accordingly. Our proposed two-level taxonomy addresses the clarity of a response in terms of the information provided for a given question (high-level) and also provides a fine-grained taxonomy of evasion techniques that relate to unclear, ambiguous responses (lower-level). We combine ChatGPT and human annotators to collect, validate and annotate discrete QA pairs from political interviews, to be used for our newly introduced response clarity task. We provide a detailed analysis and conduct several experiments with different model architectures, sizes and adaptation methods to gain insights and establish new baselines over the proposed dataset and task.

==> tables/cot.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{P{1.2cm}P{1.5cm}P{0.5cm}P{0.5cm}P{0.5cm}P{0.5cm}}
\toprule
\small Classification variant & \small Model  & \small Acc. & \small Prec. & \small Recall & \small F1    \\ \midrule
\multirow{1}{4em}{\small direct clarity}  &\small zero-shot        & \small  \underline{0.649}  & \small   \underline{0.476}   & \small  \underline{0.413}  & \small \underline{0.413}  \\
& \small standalone CoT      & \small 0.628  & \small  0.414	   & \small 0.376 	 & \small  0.368  \\ \midrule
\multirow{2}{4em}{\small evasion-based clarity} & \small zero-shot           & \small 0.640 & \small  0.507   & \small  0.497   & \small  0.482 \\
&\small standalone CoT          & \small \underline{\textbf{0.688}}  & \small  \underline{\textbf{0.611}}  & \small  \underline{\textbf{0.514}}  & \small  \underline{\textbf{0.510}} \\ 
& \small multi CoT              & \small 0.549    & \small 0.459     & \small 0.500   & \small 0.462  \\
 \bottomrule
\end{tabular}
\caption{Results for 
%chain-of-thought 
CoT inference using ChatGPT.}
\label{tab:llm-results-cot}
\end{table}

==> tables/lora.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{P{1.2cm}P{1.5cm}P{0.5cm}P{0.5cm}P{0.5cm}P{0.5cm}}
\toprule
\small Classification strategy & \small Model  & \small Acc. & \small Prec. & \small Recall & \small F1    \\ \midrule
\multirow{2}{4em}{\small direct clarity} &  \small Llama-7b &  \small 0.500      & \small 0.455    & \small 0.546 & \small 0.466 \\
& \small Llama-13b     & \small \underline{0.621}    & \small \underline{0.580}      & \small \underline{0.721}  & \small \underline{0.602} \\\midrule
& \small Llama-13b     & \small \underline{0.621}    & \small \underline{0.580}      & \small \underline{0.721}  & \small \underline{0.602} \\\midrule
\multirow{5}{4em}{\small evasion-based clarity} & \small Llama-7b    & \small 0.653    & \small 0.586    & \small 0.608 & \small 0.596 \\ 
&\small Llama-13b  & \small 0.663   & \small 0.613    & \small 0.615 & \small 0.614 \\ 
&\small Llama-70b  & \small \underline{\textbf{0.716}}   & \small \underline{\textbf{0.683}}    & \small \underline{\textbf{0.694}} & \small \underline{\textbf{0.684}} \\ %\cmidrule{2-6}
&\small Falcon-7b   & \small 0.590   & \small 0.570    & \small 0.460 & \small 0.480 \\ 
&\small Falcon-40b   & \small 0.615   & \small 0.598    & \small 0.537 & \small 0.557 \\ 
 \bottomrule
\end{tabular}
\caption{Classification results for instruction-tuned models. The best results for each strategy are \underline{underlined} and best results overall are also in \textbf{bold}.}
\label{tab:llm-results-lora}
\end{table}

==> tables/lora_v2.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{P{1.2cm}P{1.5cm}P{0.5cm}P{0.5cm}P{0.5cm}P{0.5cm}}
\toprule

\small Classification variant & \small Model  & \small Acc. & \small Prec. & \small Recall & \small F1    \\ \midrule

 \bottomrule
\end{tabular}
\caption{Results for instruction-tuned models.}
\label{tab:llm-results-lora}
\end{table}

==> tables/results_by_training.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{P{1.2cm}P{1.5cm}P{0.5cm}P{0.5cm}P{0.5cm}P{0.5cm}}
\toprule
\small Classification strategy & \small Model  & \small Acc. & \small Prec. & \small Recall & \small F1    \\ \midrule
\multirow{2}{4em}{\small direct clarity} &  \small Llama-7b &  \small 0.500      & \small 0.455    & \small 0.546 & \small 0.466 \\
& \small Llama-13b     & \small 0.621    & \small \textcolor{RoyalBlue}{0.580}      & \small \textcolor{RoyalBlue}{0.721}  & \small \textcolor{RoyalBlue}{0.602} \\\midrule
\multirow{5}{4em}{\small evasion-based clarity} & \small Llama-7b    & \small 0.653    & \small 0.586    & \small 0.608 & \small 0.596 \\ 
&\small Llama-13b  & \small 0.663   & \small 0.613    & \small 0.615 & \small 0.614 \\ 
&\small Llama-70b  & \small 0.716   & \small \textcolor{RoyalBlue}{0.683}    & \small \textcolor{RoyalBlue}{0.694} & \small \textcolor{RoyalBlue}{0.684} \\ %\cmidrule{2-6}
&\small Falcon-7b   & \small 0.590   & \small 0.570    & \small 0.460 & \small 0.480 \\ 
&\small Falcon-40b   & \small 0.615   & \small 0.598    & \small 0.537 & \small 0.557 \\ 
 \bottomrule
\end{tabular}
\caption{Classification results for instruction-tuned models (best results in \textcolor{RoyalBlue}{color}).}
\label{tab:llm-results-lora}
\end{table}


\begin{table}[h!]
\centering
\begin{tabular}{P{1.2cm}P{1.5cm}P{0.5cm}P{0.5cm}P{0.5cm}P{0.5cm}}
\toprule
\small Classification strategy & \small Model  & \small Acc. & \small Prec. & \small Recall & \small F1    \\ \midrule
\multirow{3}{4em}{\small direct clarity} &\small Llama-70b  & \small  0.467  & \small  0.429   & \small 0.235	 &  \small 0.259 \\
&\small Falcon-40b    & \small  0.240  & \small  0.252    & \small 0.247	 & \small 0.144 \\
&\small ChatGPT        & \small  \textcolor{RoyalBlue}{0.649}  & \small   0.476   & \small  0.413  & \small 0.413  \\\midrule
\multirow{3}{4em}{\small evasion-based clarity} & \small Llama-70b & \small 0.385  & \small  	0.396    & \small 0.308 & \small 0.261 \\
&\small Falcon-40b  & \small 0.618   & \small  0.365    & \small 0.387 & \small 0.375 \\
& \small ChatGPT           & \small 0.640 & \small  0.507   & \small  0.497   & \small  0.482 \\
 \bottomrule
\end{tabular}
\caption{Classification results for zero-shot (ZS) inference (best results in \textcolor{RoyalBlue}{color}).}
\label{tab:llm-results-zs}
\end{table}


\begin{table}[h!]
\centering
\begin{tabular}{P{1.2cm}P{1.5cm}P{0.5cm}P{0.5cm}P{0.5cm}P{0.5cm}}
\toprule
\small Classification strategy & \small Model  & \small Acc. & \small Prec. & \small Recall & \small F1    \\ \midrule
\multirow{1}{4em}{\small direct clarity}  &\small zero-shot        & \small  \textcolor{RoyalBlue}{0.649}  & \small   0.476   & \small  0.413  & \small 0.413  \\
& \small standalone CoT      & \small 0.628  & \small  0.414	   & \small 0.376 	 & \small  0.368  \\ \midrule
\multirow{2}{4em}{\small evasion-based clarity} & \small zero-shot           & \small 0.640 & \small  0.507   & \small  0.497   & \small  0.482 \\
&\small standalone CoT          & \small \textcolor{RoyalBlue}{0.688}  & \small  0.611  & \small  0.514  & \small  0.510 \\ 
& \small multi CoT              & \small 0.549    & \small 0.459     & \small 0.500   & \small 0.462  \\
 \bottomrule
\end{tabular}
\caption{Classification results for chain-of-thought (CoT) inference (best results in \textcolor{RoyalBlue}{color}).}
\label{tab:llm-results-cot}
\end{table}

==> tables/results_direct_clarity.tex <==


\begin{table}[h!]
\centering
\begin{tabular}{P{1.44cm}P{0.7cm}P{0.5cm}P{0.9cm}P{0.5cm}P{1.2cm}}
\hline
\small Model                        & \small Method                 & \small Acc. & \small Precision & \small Recall & \small F1  macro   \\ \hline
\small Llama-7b &  \small LoRA       & \small 0.500      & \small 0.455    & \small 0.546 & \small 0.466 \\
 \hline
\small Llama-13b & \small LoRA       & \small 0.621    & \small \textcolor{RoyalBlue}{0.580}      & \small \textcolor{RoyalBlue}{0.721}  & \small \textcolor{RoyalBlue}{0.602} \\
 \hline
\small Llama-70b & \small ZS  & \small  0.467  & \small  0.429   & \small 0.235	 &  \small 0.259 \\
\hline \hline
\small Falcon-40b & \small ZS    & \small  0.240  & \small  0.252    & \small 0.247	 & \small 0.144 \\
\hline \hline
\small ChatGPT   & \small ZS       & \small  \textcolor{RoyalBlue}{0.649}  & \small   0.476   & \small  0.413  & \small 0.413  \\
\small ChatGPT               & \small    CoT       & \small 0.628  & \small  0.414	   & \small 0.376 	 & \small  0.368  \\ \hline
\end{tabular}
\caption{Classification results on the ``clarity`` classification variant (best results in \textcolor{RoyalBlue}{color}).}
\label{tab:llm-results-1}
\end{table}

==> tables/results_evasion_based_clarity.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{P{1.44cm}P{0.7cm}P{0.5cm}P{0.9cm}P{0.5cm}P{1.2cm}}
\hline
\small Model                        & \small Method                 & \small Acc. & \small Precision & \small Recall & \small F1  macro   \\ \hline
\small Llama-7b &  \small LoRA     & \small 0.653    & \small 0.586    & \small 0.608 & \small 0.596 \\ \hline
\small Llama-13b & \small LoRA    & \small 0.663   & \small 0.613    & \small 0.615 & \small 0.614 \\ \hline

\small Llama-70b & \small ZS   & \small 0.385  & \small  	0.396    & \small 0.308 & \small 0.261 \\
\small Llama-70b & \small LoRA     & \small 0.716   & \small \textcolor{RoyalBlue}{0.683}    & \small \textcolor{RoyalBlue}{0.694} & \small \textcolor{RoyalBlue}{0.684} \\ 
\hline \hline
\small Falcon-7b & \small LoRA      & \small 0.590   & \small 0.570    & \small 0.460 & \small 0.480 \\ \hline

\small Falcon-40b & \small ZS    & \small 0.618   & \small  0.365    & \small 0.387 & \small 0.375 \\
\small Falcon-40b                   & \small LoRA            & \small 0.615   & \small 0.598    & \small 0.537 & \small 0.557 \\ 
\hline \hline

\small ChatGPT                & \small    ZS    & \small 0.640 & \small  0.507   & \small  0.497   & \small  0.482 \\

\small ChatGPT                & \small    CoT        & \small \textcolor{RoyalBlue}{0.688}  & \small  0.611  & \small  0.514  & \small  0.510 \\ \hline
\small ChatGPT           & \small CoT multi           & \small 0.549    & \small 0.459     & \small 0.500   & \small 0.462 \\
\hline
\end{tabular}
\caption{Classification results on the ``evasion`` classification variant (best results in \textcolor{RoyalBlue}{color}).}
\label{tab:llm-results-2}
\end{table}
